A Posteriori Error Estimates with Boundary Correction for a Cut Finite Element Method

In this work we study a residual based a posteriori error estimation for the CutFEM method applied to an elliptic model problem. We consider the problem with non-polygonal boundary and the analysis takes into account the geometry and data approximation on the boundary. The reliability and efficiency are theoretically proved. Moreover, constants are robust with respect to how the domain boundary cuts the mesh.

==> defs.tex <==
\newcommand{\lJump}{[\![}
\newcommand{\rJump}{]\!]}
\newcommand{\jump}[1]{[\![ #1]\!]}

\def\cT{{\mathcal T}}
\def\cE{{\mathcal E}}




\def\O{{\Omega}}
\def\o{{\omega}}

\def\bx{{\mathbf x}}
\def\by{{\mathbf y}}
\def\bz{{\mathbf z}}
\def\bn{{\mathbf n}}
\def\bp{{\mathbf p}}
\def\bnu{{\mathbf{\nu}}}







